We Need to Talk: Identifying and Overcoming Communication-Critical Scenarios for Self-Driving

In this work, we consider the task of collision-free trajectory planning for connected self-driving vehicles. We specifically consider communication-critical situations--situations where single-agent systems have blindspots that require multi-agent collaboration. To identify such situations, we propose a method which (1) simulates multi-agent perspectives from real self-driving datasets, (2) finds scenarios that are challenging for isolated agents, and (3) augments scenarios with adversarial obstructions. To overcome these challenges, we propose to extend costmap-based trajectory evaluation to a distributed multi-agent setting. We demonstrate that our bandwidth-efficient, uncertainty-aware method reduces collision rates by up to 62.5% compared to single agent baselines.

==> figure/collisionRateBars.tex <==
\begin{figure}
\vspace{1mm}
\centering
\includegraphics[width=\linewidth]{./figure/collisionRateBars.png}
\vspace*{-15pt}
\setlength{\belowcaptionskip}{-15pt}
\caption{\textbf{Task}. Collision-free planning via communication.}
\label{fig:collisionRateBars}%
\end{figure} 

==> figure/collisionRateTable3.tex <==
\begin{table*}
\vspace{5mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l||cc|cc|ccc|ccc||cc|ccc||cc}
                             &       \multicolumn{10}{c||}{Baselines}                                                                        & \multicolumn{5}{c||}{\textbf{ours: uncertainty-aware}}              & Ground Truth \\
\hline
                             &       &       &         &       &\multicolumn{3}{c|}{ego + other}&  \multicolumn{3}{c||}{ego + mostConcerned}  &         &    &  \multicolumn{3}{c||}{ego + mostConcerned}   &      \\
                             &   ego & multi & randTraj&  rand &    rand &    occ* &    ideal* &       $n=1$ &       $n=2$ &       $n=3$ &   ego & multi     &          $n=1$ &          $n=2$ &          $n=3$ &   ego* \\
\hline
top01CollisionRate           & 0.058 & 0.044 &   0.558 & 0.116 &   0.044 &   0.036 &     0.022 &       0.044 &       0.036 &       0.044 &  0.051 &    0.029 &          0.036 &          0.029 &          0.022 &   0.015\\
top01CollisionRate (rel ego) & 1.000 & 0.750 &   9.625 & 2.000 &   0.750 &   0.625 &     0.375 &       0.750 &       0.625 &       0.750 &  0.875 &    0.500 &          0.625 &          0.500 &          0.375 &   0.250\\
top10CollisionRate           & 0.143 & 0.140 &   0.508 & 0.192 &   0.136 &   0.067 &     0.064 &       0.087 &       0.078 &       0.110 &  0.156 &    0.062 &          0.078 &          0.066 &          0.055 &   0.125\\
top10CollisionRate (rel ego) & 1.000 & 0.980 &   3.558 & 1.345 &   0.954 &   0.472 &     0.447 &       0.609 &       0.548 &       0.772 &  1.091 &    0.432 &          0.548 &          0.462 &          0.386 &   0.878\\
\hline
numComLinks                  & 0.000 & 2.862 &   0.000 & 0.754 &   1.000 &   1.000 &     0.710 &       0.754 &       1.348 &       2.080 &  0.000 &    2.862 &          0.754 &          1.348 &          2.080 &   0.000\\
\end{tabular}
}
\setlength{\belowcaptionskip}{-15pt}
\caption{\textbf{Top-$k$ collision rate with $n$-agent communication}.  This table shows the collision rates of our method compared to a random sampling baseline.  The numbers in brackets show the percent change in collision rate as compared to the single-agent ($n=1$) performance.}
\label{tab:collisionRateTable}
\end{table*}


==> figure/collisionRateTable4.tex <==
\begin{table*}
\vspace{5mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccccccccc}
                             &        &        &          &        &          &          &            &              &              &              & \multicolumn{5}{c}{ours: uncertainty-aware}                                  &    &  \\
                             &        &        &          &        &      \multicolumn{3}{c}{ego + other}&  \multicolumn{3}{c}{ego + mostConcerned}      &         &           &  \multicolumn{3}{c}{ego + mostConcerned}               & \multicolumn{2}{c}{Ground Truth} \\
                             &    ego &  multi & randTraj &   rand &     rand &     occ* &     ideal* &        $n=1$ &        $n=2$ &        $n=3$ &     ego & multi     &           $n=1$ &           $n=2$ &           $n=3$ &      ego* &    multi*\\
\hline
top01CollisionRate           & 0.0580 & 0.0435 &   0.5580 & 0.1159 &   0.0435 &   0.0362 &     0.0217 &       0.0435 &       0.0362 &       0.0435 &  0.0507 &    0.0290 &          0.0362 &          0.0290 &          0.0217 &   0.0145 &     0.0000\\
top01CollisionRate (rel ego) & 1.0000 & 0.7500 &   9.6250 & 2.0000 &   0.7500 &   0.6250 &     0.3750 &       0.7500 &       0.6250 &       0.7500 &  0.8750 &    0.5000 &          0.6250 &          0.5000 &          0.3750 &   0.2500 &     0.0000\\
top10CollisionRate           & 0.1428 & 0.1399 &   0.5080 & 0.1920 &   0.1362 &   0.0674 &     0.0638 &       0.0870 &       0.0783 &       0.1101 &  0.1558 &    0.0616 &          0.0783 &          0.0659 &          0.0551 &   0.1254 &     0.0000\\
top10CollisionRate (rel ego) & 1.0000 & 0.9797 &   3.5584 & 1.3452 &   0.9543 &   0.4721 &     0.4467 &       0.6091 &       0.5482 &       0.7716 &  1.0914 &    0.4315 &          0.5482 &          0.4619 &          0.3858 &   0.8782 &     0.0000\\
numComLinks                  & 0.0000 & 2.8623 &   0.0000 & 0.7536 &   1.0000 &   1.0000 &     0.7101 &       0.7536 &       1.3478 &       2.0797 &  0.0000 &    2.8623 &          0.7536 &          1.3478 &          2.0797 &   0.0000 &     2.8623\\
\end{tabular}
}
\setlength{\belowcaptionskip}{-15pt}
\caption{\textbf{Top-$k$ collision rate with $n$-agent communication}.  This table shows the collision rates of our method compared to a random sampling baseline.  The numbers in brackets show the percent change in collision rate as compared to the single-agent ($n=1$) performance.}
\label{tab:collisionRateTable}
\end{table*}


==> figure/collisionRateTableFractions.tex <==
\begin{table*}
\vspace{5mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccl||cc|cc||c}
                            &                           &                 &           \multicolumn{4}{c|}{Top-$k$ Collision Rate}                                               & Communication\\
                           &                            &                 &              $k=1$ &                  (rel to ego) &             $k=10$ &                  (rel to ego) & Links\\
\hline
Ego Only                   & ego                        &                 &              0.058 &                        1.000 &              0.143 &                        1.000 &       0.000\\
                           & randTraj                   &                 &              0.486 &                        8.375 &              0.522 &                        3.655 &       0.000\\
                           & rand                       &                 &              0.080 &                        1.375 &              0.223 &                        1.563 &       0.783\\
\midrule
Ours: Bandwidth-Efficient  & ego+rand                   &                 &              0.036 &                        0.625 &              0.128 &                        0.898 &       1.000\\
Trajectory Exchange        & ego+occ*                   &                 &              0.036 &                        0.625 &              0.067 &                        0.472 &       1.000\\
                           & ego+ideal*                 &                 &              0.022 &                        0.375 &              0.064 &                        0.447 &       0.710\\
                           & multi                      &                 &              0.043 &                        0.750 &              0.140 &                        0.980 &       2.862\\
\cmidrule(lr){2-8}                           
                           & ego+concern                & $N=1$           &              0.043 &                        0.750 &              0.087 &                        0.609 &       0.754\\
                           &                            & $N=2$           &              0.036 &                        0.625 &              0.078 &                        0.548 &       1.348\\
                           &                            & $N=3$           &              0.043 &                        0.750 &              0.110 &                        0.772 &       2.080\\
\midrule
Ours: Uncertainty-Aware    & ego                        &                 &              0.051 &                        0.875 &              0.156 &                        1.091 &       0.000\\
Trajectory Exchange        & multi                      &                 &              0.029 &                        0.500 &              0.062 &                        0.431 &       2.862\\
 \cmidrule(lr){2-8}                           
                           & ego+concern                & $N=1$           &              0.036 &                        0.625 &              0.078 &                        0.548 &       0.754\\
                           &                            & $N=2$           &              0.029 &                        0.500 &              0.066 &                        0.462 &       1.348\\
                           &                            & $N=3$           &              0.022 &                        0.375 &              0.055 &                        0.386 &       2.080\\
\midrule
Ground Truth               & ego*                       &                 &              0.014 &                        0.250 &              0.125 &                        0.878 &       0.000\\
\end{tabular}
}
\setlength{\belowcaptionskip}{-15pt}
\caption{\textbf{Top-$k$ collision rate with $n$-agent communication}.  This table shows the collision rates of our method compared to a random sampling baseline.  The numbers in brackets show the percent change in collision rate as compared to the single-agent ($n=1$) performance.}
\label{tab:collisionRateTable}
\end{table*}

==> figure/comCritFrequencyAugmented.tex <==
\begin{figure}
\vspace{1mm}
\centering
\includegraphics[scale=0.5]{figure/comCritFrequencyAugmented.png}
% \vspace*{-15pt}
% \setlength{\belowcaptionskip}{-15pt}
\caption{\textbf{Task}. Collision-free planning via communication.}
\label{fig:frequency}%
\end{figure} 



==> figure/comCritFrequencyNatural.tex <==
\begin{figure*}
\vspace{1mm}
\centering
\includegraphics[scale=0.5]{figure/comCritFrequencyNatural.png}
\caption{\textbf{Task}. Collision-free planning via communication.}
\label{fig:frequency}%
\end{figure*} 


